Development of Fault Tolerant MAS with Cooperative Error Recovery by Refinement in Event-B

Designing fault tolerance mechanisms for multi-agent systems is a notoriously difficult task. In this paper we present an approach to formal development of a fault tolerant multi-agent system by refinement in Event-B. We demonstrate how to formally specify cooperative error recovery and dynamic reconfiguration in Event-B. Moreover, we discuss how to express and verify essential properties of a fault tolerant multi-agent system while refining it. The approach is illustrated by a case study - a multi-robotic system.

==> convheader.tex <==

\newcommand{\fMODE} 			{\mathrm{MODE}}
\newcommand{\fMORDER} 			{\mathrm{ORDER}}
\newcommand{\fERROR} 			{\mathrm{ERROR}}
\newcommand{\fNOERROR} 			{\mathrm{NoError}}
\newcommand{\fINITMODE} 		{\mathrm{InitMode}}
\newcommand{\fMode}[1] 			{\mathrm{#1}}
\newcommand{\fConst}[1] 		{\mathrm{#1}}

\newcommand{\kG}[1]					{{\bf\textsc{#1}}}
\newcommand{\kB}[1]					{{\sf #1}}

\newcommand{\kwSYSTEM}			{machine}
\newcommand{\kwINTERFACE}		{interface}
\newcommand{\kwREFINEMENT}		{refinement}
\newcommand{\kwVARIABLES}		{variables}
\newcommand{\kwINVARIANT}		{invariant}
\newcommand{\kwINITIALISATION}	{initialisation}
\newcommand{\kwEVENTS}			{events}
\newcommand{\kwOPERATIONS}		{operations}
\newcommand{\kwPARAMETERS}		{parameters}
\newcommand{\kwPROPERTIES}		{properties}
\newcommand{\kwANY}				{any}
\newcommand{\kwWHERE}			{where}
\newcommand{\kwTHEN}			{then}
\newcommand{\kwWHEN}			{when}
\newcommand{\kwSEES}			{sees}
\newcommand{\kwSKIP}			{skip}
\newcommand{\kwEND}				{end}
\newcommand{\kwBEGIN}			{begin}
\newcommand{\kwPRE}				{pre}
\newcommand{\kwPOST}			{post}
\newcommand{\kwREFINES}			{refines}
\newcommand{\LABEL}[1]			{\mathrm{#1}:~}

\newcommand{\EventBSnippet}[1] {
	{\footnotesize{
	$
	\begin{array}{@{}l} #1 \end{array}
	$
	}}
}


\newcommand{\EventBSystem}[2] {
	{\footnotesize{
	$
	\begin{array}{@{}l}
		\kG{\kwSYSTEM} ~ \kB{#1} \\
		\quad \begin{array}{@{}l} #2 \end{array} \\
		\kG{\kwEND}
	\end{array}
	$
	}}
}


\newcommand{\EventBContext}[2] {
	{\footnotesize{
	$
	\begin{array}{@{}l}
		\kG{context} ~ \kB{#1} \\
		\quad \begin{array}{@{}l} #2 \end{array} \\
		\kG{\kwEND}
	\end{array}
	$
	}}
}

\newcommand{\EventBContextd}[2] {
	{\footnotesize{
	$
	\begin{array}{@{}l}
		\kG{context} ~ \kB{#1} \\
		\quad \begin{array}{@{}l} #2 \end{array} \\
		%\kG{$\cdots$}
	\end{array}
	$
	}}
}


\newcommand{\EventBInterface}[2] {
	{\footnotesize{
	$
	\begin{array}{@{}l}
		\kG{\kwINTERFACE} ~ \kB{#1} \\
		\quad \begin{array}{@{}l} #2 \end{array} \\
		\kG{\kwEND}
	\end{array}
	$
	}}
}

\newcommand{\EventBRefinement}[2] {
	{\footnotesize{
	$
	\begin{array}{@{}l}
		\kG{\kwREFINEMENT} ~ \kB{#1} \\
		\quad \begin{array}{@{}l} #2 \end{array} \\
		\kG{\kwEND}
	\end{array}
	$
	}}
}




\newcommand{\EventBTemplate}[2] {
	$
	\begin{array}{@{}l}
		\kG{\kwTEMPLATE} ~ \kB{#1} \\
		\begin{array}{@{}l} #2 \end{array}
	\end{array}
	$
}


\newcommand{\EventBTemplateB}[2] {
	$\left (
	\begin{array}{@{}l}
		\kG{\kwTEMPLATE} ~ \kB{#1} \\
		\begin{array}{@{}l} #2 \end{array}
	\end{array}
	\right )$
}

\newcommand{\EventBGroup}[2] {


		\kG{group} ~ \kB{#1} ~ \kG{begin}\\
		\begin{array}{@{}l} \quad \begin{array}{rll} #2 \end{array} \end{array} \\
		\kG{end} \\
}

\newcommand{\EventBCont}[1] {
	{\footnotesize{
	$
	\begin{array}{@{}l}
		\begin{array}{@{}l} \quad \begin{array}{rll} #1 \end{array} \end{array}
	\end{array}
	$}}
}


\newcommand{\EventBE}[1] {
	\begin{array}{@{}l} \quad \begin{array}{lll} #1 \end{array} \end{array}
}


\newcommand{\EventBRefines}[1] {
	\kG{\kwREFINES} ~ \kB{#1} \\
}


\newcommand{\EventBImplements}[1] {
	\kG{implements} ~ \kB{#1} \\
}


\newcommand{\EventBExtends}[1] {
	\kG{extends} ~ \kB{#1} \\
}

\newcommand{\EventBSees}[1] {
	\kG{\kwSEES} ~ \kB{#1} \\
}


\newcommand{\EventBVars}[1] {
	\kG{\kwVARIABLES} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\EventBConstantsC}[1] {
	\kG{constants} ~ #1 \\
}

\newcommand{\EventBAxioms}[1] {
	\kG{axioms} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\EventBFlow}[1] {
	\kG{\kwFLOW} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\EventBVarsC}[1] {
	\kG{\kwVARIABLES} ~ #1 \\
}

%\newcommand{\EventBConstantsC}[1] {
%	\kG{constants} ~ #1 \\
%}

%\newcommand{\EventBAxioms}[1] {
%	\kG{axioms} ~ #1 \\
%}

\newcommand{\EventBParamsC}[1] {
	\kG{\kwPARAMETERS} ~ #1 \\
}

\newcommand{\EventBProperties}[1] {
	\kG{\kwPROPERTIES} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\EventBInv}[1] {
	\kG{\kwINVARIANT} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\EventBInvC}[1] {
	\kG{\kwINVARIANT} ~ #1 \\
}

\newcommand{\EventBFaultsC}[1] {
	\kG{faults} ~ #1 \\
}

\newcommand{\EventBUsesC}[1] {
	\kG{uses} ~ \kB{#1} \\
}

\newcommand{\EventBUses}[2] {
	\kG{uses} ~ \kB{#1} \\
	\quad \begin{array}{l} #2 \end{array} \\
}


\newcommand{\EventBFaults}[1] {
	\kG{faults} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\Fault}[2] {
	\kB{#1} : #2 \\
}



\newcommand{\EventBInit}[1] {
	\kG{\kwINITIALISATION} \\
	\quad \begin{array}{l} #1 \end{array} \\
}

\newcommand{\EventBInitC}[1] {
	\kG{\kwINITIALISATION} ~ #1 \\
}

\newcommand{\EventBEvents}[1] {
	\kG{\kwEVENTS} \\
	\quad \begin{array}{lll} #1 \end{array} \\
}



\newcommand{\EventBOperations}[1] {
	\kG{\kwOPERATIONS} \\
	\quad \begin{array}{lll} #1 \end{array} \\
}

\newcommand{\EventBEventsTwoCol}[1] {
	\kG{\kwEVENTS} \\
	\quad \begin{array}{lll} #1 \end{array} \\
}

\newcommand{\EventBContTwoCol}[1] {
	$\begin{array}{lll} #1 \end{array}$
}

\newcommand{\EventBEventsRow}[2] {
	\begin{array}{lll} #1 \end{array} & \quad & \begin{array}{lll} #2 \end{array}\\
}

\newcommand{\EventBEventsRowSpan}[1] {
	\multicolumn{3}{l}{ \begin{array}{lll} #1 \end{array} }\\
}

\newcommand{\EventBAny}[4] {
  \kB{#1} & = 	& 	\kG{\kwANY} ~ #2 ~ \kG{\kwWHERE} \\
			  && 	\quad \begin{array}{l} #3 \end{array} \\
			  && 	\kG{\kwTHEN} \\
			  && 	\quad \begin{array}{l} #4 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBAnyOperation}[4] {
  \kB{#1} & = 	& 	\kG{\kwANY} ~ #2 ~ \kG{\kwPRE} \\
			  && 	\quad \begin{array}{l} #3 \end{array} \\
			  && 	\kG{\kwPOST} \\
			  && 	\quad \begin{array}{l} #4 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBAnyRefines}[5] {
  \kB{#1} ~ \kG{refines} ~  #2 & = 	& 	\kG{\kwANY} ~ #3 ~ \kG{\kwWHERE} \\
			  && 	\quad \begin{array}{l} #4 \end{array} \\
			  && 	\kG{\kwTHEN} \\
			  && 	\quad \begin{array}{l} #5 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBAnyC}[4] {
   \kB{#1} & = 	& 	\kG{\kwANY} ~ #2 ~ \kG{\kwWHERE} ~ #3 ~ \kG{\kwTHEN} ~#4~ \kG{\kwEND} \\
}


\newcommand{\EventBWhen}[3] {
   \kB{#1} & = 	& \kG{\kwWHEN} \\ 
			  && 	\quad \begin{array}{l} #2 \end{array} \\
			  && 	\kG{\kwTHEN} \\
			  && 	\quad \begin{array}{l} #3 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBWhenOperation}[3] {
   \kB{#1} & = 	& \kG{\kwPRE} \\ 
			  && 	\quad \begin{array}{l} #2 \end{array} \\
			  && 	\kG{\kwPOST} \\
			  && 	\quad \begin{array}{l} #3 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBWhenRefines}[4] {
  \kB{#1} ~ \kG{ref} ~ #2 & = 	& \kG{\kwWHEN} \\ 
			  && 	\quad \begin{array}{l} #3 \end{array} \\
			  && 	\kG{\kwTHEN} \\
			  && 	\quad \begin{array}{l} #4 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBWhenC}[3] {
   \kB{#1} & = 	& \kG{\kwWHEN} ~#2~ \kG{\kwTHEN} ~#3~ \kG{\kwEND} \\
}

\newcommand{\EventBWhenOperationC}[3] {
   \kB{#1} & = 	& \kG{pre} ~#2~ \kG{post} ~#3~ \kG{\kwEND} \\
}

\newcommand{\EventBBegin}[2] {
   \kB{#1} & = 	& 	\kG{\kwBEGIN} \\
			  && 	\quad \begin{array}{l} #2 \end{array} \\
			  && 	\kG{\kwEND} \\
}

\newcommand{\EventBBeginC}[2] {
   \kB{#1} & = 	& 	\kG{\kwBEGIN} ~ #2 ~ \kG{\kwEND} \\
}

\newcommand{\EventBSkip}[1] {
   \kB{#1} & = 	& 	\kG{\kwSKIP} \\
}

\newcommand{\EventBSF}[2] {
   \kB{#1} & = 	& 	#2 \\
}



